Fully Statistical Neural Belief Tracking

This paper proposes an improvement to the existing data-driven Neural Belief Tracking (NBT) framework for Dialogue State Tracking (DST). The existing NBT model uses a hand-crafted belief state update mechanism which involves an expensive manual retuning step whenever the model is deployed to a new dialogue domain. We show that this update mechanism can be learned jointly with the semantic decoding and context modelling parts of the NBT model, eliminating the last rule-based module from this DST framework. We propose two different statistical update mechanisms and show that dialogue dynamics can be modelled with a very small number of additional model parameters. In our DST evaluation over three languages, we show that this model achieves competitive performance and provides a robust framework for building resource-light DST models.

==> notes-work.tex <==
TOP WOZ Performance: 

{
    "food": 0.908, 
    "joint": 0.861, 
    "price range": 0.944, 
    "request": 0.761, 
    "area": 0.948
}

New WOZ performance: 

{
    "dstc2 food": 0.874, 
    "dstc2 price range": 0.939, 
    "request": 0.0, 
    "joint": 0.815, 
    "dstc2 area": 0.913
}

